Testing and Debugging Quantum Circuits

This paper introduces a process framework for debugging quantum circuits, focusing on three distinct types of circuit blocks: Amplitude Permutation, Phase Modulation, and Amplitude Redistribution circuit blocks. Our research addresses the critical need for specialized debugging approaches tailored to the unique properties of each circuit type. For Amplitude Permutation Circuits, we propose techniques to correct amplitude permutations mimicking classical operations. In phase modulation circuits, our proposed strategy targets the precise calibration of phase alterations essential for quantum computations. The most complex Amplitude Redistribution Circuits demand advanced methods to adjust probability amplitudes. This research bridges a vital gap in current methodologies and lays the groundwork for future advancements in quantum circuit debugging. Our contributions are twofold: We present a comprehensive unit testing tool (Cirquo) and debugging approaches tailored to the unique demands of quantum computing, and we provide empirical evidence of its effectiveness in optimizing quantum circuit performance. This work is a crucial step toward realizing robust quantum computing systems and their applications in various domains.

==> Content/extras.tex <==


\begin{lstlisting}[language=Python, caption=Test vectors for the 3-qubit Dicke state with Hamming distance 2., label=test_ds]
{
'name': 'test 0', 'input': [(1+0j), 0j, 0j, 0j, 0j, 0j, 0j, 0j], 'expected_output': [0j, 0j, 0j, (0.577+0j), 0j, (0.577+0j), (0.577+0j), 0j]
}
{
'name': 'test 1', 'input': [0j, 0j, 0j, 0j, 0j, 0j, 0j, (1+0j)], 'expected_output': [0j, (0.707+0j), (-0.707+0j), 0j, 0j, 0j, 0j, 0j]
}
{
'name': 'test +', 'input': [(0.353+0j), (0.353+0j), (0.353+0j), (0.353+0j), (0.353+0j), (0.353+0j), (0.353+0j), (0.353+0j)], 'expected_output': [(0.353+0j), (0.598+0j), (0.098+0j), (0.606+0j), (-0.084+0j), (-0.056+0j), (0.062+0j), (0.353+0j)]
}
{
'name': 'test -', 'input': [(0.353+0j), (-0.353+0j), (-0.353+0j), (0.353+0j), (-0.353+0j), (0.353+0j), (0.353+0j), (-0.353+0j)], 'expected_output': [(0.353+0j), (-0.598+0j), (-0.098+0j), (0.606+0j), (0.084+0j), (-0.056+0j), (0.062+0j), (-0.353+0j)]
}
{
'name': 'test i', 'input': [(0.353+0j), 0.353j, 0.353j, (-0.353+0j), 0.353j, (-0.353+0j), (-0.353+0j), -0.353j], 'expected_output': [(-0.353+0j), 0.098j, 0.598j, (-0.198+0j), -0.084j, (0.465+0j), (0.345+0j), 0.353j]
}
{
'name': 'test -i', 'input': [(0.353+0j), -0.353j, -0.353j, (-0.353+0j), -0.353j, (-0.353+0j), (-0.353+0j), 0.353j], 'expected_output': [(-0.353+0j), -0.098j, -0.598j, (-0.198+0j), 0.084j, (0.465+0j), (0.345+0j), -0.353j]
}
\end{lstlisting} 



\begin{lstlisting}[language=bash, caption=Test results when running the test vectors of the three-qubit W state program with amplitude bug corresponding to Fig.~\ref{3wc_bs}-b., label=ws_res-b]
W State Test 1:
Result:  FAIL
Input:  1.00|000>
Output:  1.00|000>
Expected Output:  0.58|001> + 0.58|010> + 0.58|100>

W State Test 2:
Result:  FAIL
Input:  1.00|111>
Output:  -0.41|001> + 0.20|010> + 0.61|011> + 0.20|100> + -0.61|101>
Expected Output:  0.71|011> + -0.71|101>
\end{lstlisting}





\section{The Sources and Effect of Bugs in Quantum Programs}
\label{sec:bugs}


Most work done around the field of testing and debugging quantum software mainly focused on finding patterns in quantum bugs and collecting frequent bugs. Since understanding the flow of quantum programs and the causes of errors is essential for the ability to debug quantum circuits, researchers focused on categorizing reproducible bugs in quantum programs~\cite{zhao2021bugs4q,campos2021qbugs,luo2022comprehensive}. In these studies, researchers found that bugs in quantum programs can occur for two reasons: either the package used or the developer's implementation. Package-related errors occur due to a fault in the implementation of the core functionalities of the package, such as deprecation and mistakes in the data handling. On the other hand, bugs introduced by the developer cover incidents such as the wrong type/ordering of the gates or misuse of the package functions.

%A categorization of the source of quantum bugs that might occur when implementing quantum algorithms is to divide them into 4 categories, bugs due to the package used to implement the algorithm, bugs due to a fault in the logic of the application, math-related bugs, or bugs due to an error outside of the above reasons. 

%Because the package used to implement quantum programs can introduce some errors to the programs~\cite{10.1145/3527330, 10172716} conducted work on these types of bugs and how they can affect quantum programs.

In the work done by Luo et al.~\cite{luo2022comprehensive}, 96 faulty quantum programs were categorized based on the source of the error that occurred in them. 35 of the errors were related to the package, while 61 were introduced by the developer. 
We collected an additional 73 faulty programs from the same sources (Stack Overflow, Stack Exchange, and GitHub) and then classified them into four categories: 
\begin{itemize}
    \item \textbf{Job handling errors} which include transpilation, decomposition, and simulation errors and those related to the package implementation. %These types of bugs are not introduced by the programmer and may cause a correct implementation not to work properly.  
    \item \textbf{Classical data post-processing errors} which include misunderstanding/ wrong interpretation of the data or a mistake in parameterizing the circuit. %This category of bugs is about the different ways the results can be mistakenly interpreted by the programmer. A common example of this bug is the little Indian vs. big Indian representation of the qubits.
    \item \textbf{Classical bugs} include typos and mishandling of functions, such as missing attributes and confusing data types. This type of bugs is not quantum-specific. They also occur in classical programs, and though these bugs may lead to false circuit results, fixing them does not require any quantum knowledge.
    \item \textbf{Quantum circuit bugs} These are the bugs that will cause difficulties in developing larger quantum software in the future. Quantum circuit bugs include missing or extra gates, applying a gate to the wrong qubit, wrong gate order, initialization error, wrong phase, or using the wrong gates.
\end{itemize}

\if 0
\begin{table}[]
\centering
\caption{The count of bugs causing syntax errors is based on whether they are caused by the package or the user.}
\label{tab:syntax}
\begin{tabular}{ccc|c}
\cline{2-3}
\multicolumn{1}{c|}{}                              & \multicolumn{2}{c|}{\cellcolor[HTML]{FFCC67}Cause Syntax error?} &                          \\ \cline{2-4} 
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCC67}Yes} & \cellcolor[HTML]{FFCC67}No & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCC67}Sum} \\ \hline
\multicolumn{1}{|c|}{\cellcolor[HTML]{68CBD0}package}  & \multicolumn{1}{c|}{35}      & 8                                 & \multicolumn{1}{c|}{43}  \\ \hline
\multicolumn{1}{|c|}{\cellcolor[HTML]{68CBD0}User} & \multicolumn{1}{c|}{39}      & 41                                & \multicolumn{1}{c|}{80}  \\ \hline
                                                   & \multicolumn{1}{c|}{}        & \cellcolor[HTML]{FD6864}Total     & \multicolumn{1}{c|}{123} \\ \cline{3-4} 
\end{tabular}
\end{table}
\fi 

%Understanding the type of bugs that can occur in quantum programs is essential to the process of debugging and testing quantum programs. A simple differentiation we can make here is: How many of these bugs cause a syntax error? If a syntax error arises, locating the bug will be easier, and fixing it as well. 

Moreover, if we consider the categorization above, we can refer to the first three categories as non-quantum-specific bugs and the last category as quantum bugs. Those categories include bugs that could also occur in classical programming; hence, we can approach debugging them as we do classically. Table~\ref{tab:bugs} shows the distribution of the bugs based on their source and category. %Another important note about such bugs is that they often cause syntax errors, making them easier to locate and fix.

\if 0
Let us consider the non-quantum-specific errors first. These bugs are introduced by the package used, misuse of that package by the programmer, or misinterpretation of the results. Bugs introduced by the package used include errors due to deprecation or compatibility between the package and its dependencies. These errors are often captured during compilation time.  

\begin{lstlisting}[language=Python, caption=An example of non-quantum-specific bug due to misuse of the package by the programmer~\cite{VishVish}., label=user_misuse]
from qiskit.providers.aer import QasmSimulator
# Create a quantum circuit
qc = QuantumCircuit(2, 2)
qc.h(0)
qc.cx(0, 1)
qc.measure([0, 1], [0, 1])
# Get the Qasm simulator and set the backend options
aer_qasm_simulator = Aer.get_backend(              'qasm_simulator')
# Set the backend options, method set to statevector
options = {'method': 'statevector', 'memory' : True, 'shots':10}
# Execute circuit using the backend options created
job = execute(qc, backend_simulator, backend_options=options)
result = job.result()
# Pull the memory slots for the circuit
memory = result.get_memory(qc)
# Print the results from the memory slots
print('Memory results: ', memory)
\end{lstlisting} 

In Listing~\ref{package_bug}, we can see an example of a piece of code that produced an error due to the deprecation of the function \textit{Shor} in the recent versions of Qiskit~\cite{Anita}. Another example of a non-quantum-specific bug~\cite{VishVish} can be seen in Listing~\ref{user_misuse}, where this piece of code produces an error because the programmer used the wrong parameters when choosing a backend to execute the circuit. Finally, the programmer can implement an algorithm correctly and have no issues due to the package, yet misinterprets the results and thinks they are incorrect; this is often due to confusing little and big Indian representations of the qubits.

\begin{lstlisting}[language=Python, caption=A simple example of a bug due to the package (Qiskit) deprecation of the Shor function~\cite{Anita}., label=package_bug]
from qiskit import Aer
from qiskit.utils import QuantumInstance
from qiskit.algorithms import Shor

N = 15
backend = Aer.get_backend('aer_simulator')
quantum_instance = QuantumInstance(backend, shots=1024)
shor = Shor(quantum_instance=quantum_instance)
result = shor.factor(N)
print(f"The list of factors of {N} as computed by the Shor's algorithm is {result.factors[0]}.")
\end{lstlisting} 
\fi

% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\centering
\caption{Categorizing the bugs collected from StackExchange and StackOverflow based on their type and cause.}
\label{tab:bugs}
\begin{tabular}{c|cc|l}
\cline{2-3}
                                                                          & \multicolumn{2}{c|}{\cellcolor[HTML]{68CBD0}Bug Source} &                          \\ \cline{1-3}
\multicolumn{1}{|c|}{\cellcolor[HTML]{68CBD0}Bug Type} & \multicolumn{1}{c|}{\cellcolor[HTML]{68CBD0}Due to package} & \cellcolor[HTML]{68CBD0}Due to User &  \\ \cline{1-3}
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFCC67}Classical Data Post-processing} & \multicolumn{1}{c|}{11}               & 15              &                          \\ \cline{1-3}
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFCC67}Classical Bugs}                 & \multicolumn{1}{c|}{4}                & 24              &                          \\ \cline{1-3}
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFCC67}Quantum Circuit}                & \multicolumn{1}{c|}{1}                & 37              &                          \\ \cline{1-3}
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFCC67}Job Handling}                   & \multicolumn{1}{c|}{27}               & 4               &                          \\ \hline
\multicolumn{1}{|c|}{\cellcolor[HTML]{FD6864}Total}                          & \multicolumn{1}{c|}{43}               & 80              & \multicolumn{1}{l|}{123} \\ \hline
\end{tabular}
\end{table}

Before we take a closer look at the quantum circuit bugs, we need first to have a clear definition of what a quantum bug is. A quantum bug, at a high level, is an error in creating the correct interference patterns. Which can occur due to different causes depending on the algorithm the programmer is implementing. For example, suppose the programmer is writing an implementation for Grover or Shor's algorithms. In that case, the cause of interference pattern errors can be due to failure in cleaning or detangling the ancilla qubits, a mistake in marking the correct state/s, an improper implementation of the diffusion operator, or, possibly, a combination of all the above. On the other hand, if the programmer is implementing a quantum chemistry or physics simulation, the errors are "mathematical" due to using the wrong Hamiltonian. Moreover, if the programmer is implementing a variational quantum algorithm (VQA), such as Variational QUantum Eigensolver (VQE) or Quantum Approximate Optimization Algorithm (QAOA), then the source of error could be the wrong ansatz or a mistake in setting the parameters of the classical optimizer. 
Though all these bugs manifest as wrong interference patters, on a circuit level, all these types of errors will translate to using the wrong gate types/ order, applying the wrong phases, or a combination of both. 
%Examining these bugs closer generated by programmers, it is essential to recognize that the repercussions of these bugs can vary significantly depending on the specific application of the algorithm chosen and how it is implemented. 
These bugs will either throw a runtime exception which is easy to catch and fix, or lead to the wrong answer making them potentially more challenging to locate and fix.
We can classify these bugs into several categories:

\begin{enumerate}
    \item \textbf{Initialization Bugs}: These occur at the beginning stages, such as:
    \begin{itemize}
        \item \textit{State Preparation}: Errors occur while setting up the initial state of the quantum system.
        \item \textit{Parameter Initialization}: Mistakes in initializing the parameters necessary for the quantum algorithm.
    \end{itemize}
    \item \textbf{Gate-related Bugs}: This category includes any error arising due to gates such as:
    \begin{itemize}
        \item \textit{Incorrect Gate Sequence}: Errors due to the application of gates in an incorrect order.
        \item \textit{Unwanted Gate Inclusion}: Extra gates are not necessary for the specific computation.
        \item \textit{Wrong Qubit Targeting}: Applying gates to the wrong qubits.
    \end{itemize}
    \item \textbf{Quantum Logic Bugs}: This category includes bugs not due to the initial state or the order/ type of gates, such as:  
    \begin{itemize}
        \item \textit{Algorithmic Misinterpretation}: Errors arising from incorrect understanding or implementation of the algorithm.
        \item \textit{Phase Setting}: Mistakes in setting the correct phase for certain operations.
        \item \textit{Measurement Location}: Errors due to applying the measurement operation at the wrong time in the circuit.
    \end{itemize}
\end{enumerate}

%Add the bug example here!!!!!!!!!!!!!!!!!!!!!!!!
%By understanding and categorizing these bugs, we can develop more robust strategies to identify and mitigate them.

Let us take a closer look at each of these categories, starting with initialization bugs. These bugs indicate that the programmer made a mistake in the initial state required to execute the algorithm correctly.
An example of that would be "forgetting" to prepare the qubits in state $\vert+\rangle$ when constructing a cluster state~\cite{NIELSEN2006147} as can be seen in Listing~\ref{cluster_bug}. Moreover, mistakes in the state preparation when implementing different algorithms, such as Grover and Shor algorithms, are considered initialization bugs. 

\begin{lstlisting}[language=Python, caption=A Python and Qiskit implementation of 1D cluster states missing the initialization of the qubits to the $\vert+\rangle$ state by applying H gate to all qubits before the CZ gates., label=cluster_bug]
from qiskit import QuantumCircuit
def create_cluster_state(n_qubits: int) -> QuantumCircuit:
    """Create a cluster state for the given number of qubits."""    
    # Initialize a quantum circuit with the specified number of qubits
    qc = QuantumCircuit(n_qubits)
    # Apply CZ gates between neighboring qubits to create the 1D cluster state
    for i in range(n_qubits - 1):
        qc.cz(i, i+1)    
    return qc

n_qubits = 4
cluster_circuit = create_cluster_state(n_qubits)
\end{lstlisting} 

Another common category of quantum-specific bugs is those that involve gates. This includes applying gates to the wrong qubits or in the wrong order. 
%In addition to missing adding a gate or adding an extra gate.
An example of that will be discussed in detail in Section~\ref{sec:test}.

The final category of quantum-specific bugs is what we refer to as quantum-logic bugs. This category includes bugs such as phase errors due to using the wrong phase or making a mistake in translating an algorithm into code. An example of such a bug is further discussed in Section~\ref{sec:test}.% when we address an example of testing and debugging a full-quantum circuit.







==============================================================


\subsection{Examining the individual slices}
Once we obtain the smaller circuits from the slicer---or already have the circuit---and know its categorization, we need to start testing it and observe its behavior. Cirquo offers two testing functions, \texttt{pClassTester} and \texttt{fQuantTester}, to run tests on pseudo-classical and full-quantum circuits, respectively. 

The \texttt{pClassTester} allows the programmer to pass the test cases as a list of classical values of the qubits---that is, $0$ or $1$---that input is converted to a state vector before running the circuit. That is to make testing the classical circuits more intuitive than how we test classical software. For example, if a programmer needs to test a quantum full-adder circuit and wants to test the circuit results if the inputs were $1,1$ and $1$, they can pass the \texttt{pClassTester} a list [1,1,1]. More details on testing pseudo-classical circuits, generally, and the full-adder precisely are in Section~\ref{sec:test}.

The \texttt{fQuantTester} takes a list of state vectors and their corresponding outputs and runs the circuit accordingly. Testing full-quantum circuits can be challenging; hence, programmers often do not know how to test these circuits. Cirquo also contains implementation and sample test vectors for common building blocks in quantum algorithms.

If a programmer wants to test a full-quantum circuit, they can describe the inputs and corresponding outputs as state vectors. For example, if we were to test a simple Bell pair generator, we would need to format the input and output tests as state vectors. So, in the case of a 2-qubit Bell pair generator circuit consisting of a Hadamard gate and a CNOT gate, if the initial state of the qubits is $\vert0\rangle$ and $\vert0\rangle$, then the results should be $0.71\vert00\rangle + 0.71\vert11\rangle$. To prepare that for the tester, the input state will be $[1,0,0,0]$ because the state vector of 2 qubits consists of $2^2$ cases. More details on the construction of tests for full-quantum circuits are given in Section~\ref{sec:test}.
In addition to the test samples, programmers can also use the pre-defined functions of these building blocks to assist them in constructing their circuits. 



\subsection{Gate tracking}
Understanding how the circuit behaves is the key to making the testing and debugging process more efficient. Therefore, Cirquo offers some functions that provide information to make testing the circuit a better experience for the programmer. 

When an error occurs while executing a circuit on actual hardware, it is often due to the hardware (machine-related) or the quantum logic (algorithm and implementation). Machine-related errors are low-level hardware-specific faults such as gate errors, readout errors, thermal relaxation errors, measurement errors, etc.~\cite{tannu2019mitigating, PhysRevLett.119.180509, PhysRevX.8.031027}. Fixing these errors requires implementing quantum error correction and some efficient error minimizing technique~\cite{PhysRevX.7.021050} (or being very lucky on a given run). However, when a circuit is simulated (or we can be certain that the error is not due to the hardware), the difficulty in fixing these errors arises from the nature of quantum algorithms.

Most quantum algorithms select an outcome from a probability distribution at the end of a run partly because they use superposition, entanglement, and interference. Thus, isolating the circuit section containing the error requires careful reasoning and narrowing down operations to make the error as reproducible and visible as possible.

One aspect of this is the need for the programmer to work both forward and backward through the toolchain, examining the circuit at the gate level and the higher-level functions that generated the circuit. Cirquo allows the programmer to track where each gate was added to the circuit in the code.\\

The complete list of Cirquo's functions is in the appendix.

===============================================================
\subsection{Generating Test Vectors}
%One of the key elements missing in all quantum software today is testing, more particularly creating test vectors. Though some tools offer unit testing for quantum programs, they leave it completely to the programmer to generate test vectors.

Cirquo offers functions to implement some commonly used subroutines in quantum algorithms and some test vectors for them to ease the load off the programmer. Cirquo's test vectors mainly use the \textbf{statevector} to represent the input/output test case pairs. Since Cirquo is built on Qiskit, if the programmer wants to use the QASM simulator to test the circuit, they can add the \textit{state\_vector} as a backend option in the \textit{execute} function \texttt{job = execute(qc, backend, backend\_options = {'method': 'statevector'})}. From there, they can obtain the statevector using the \texttt{get\_statevector} method as \texttt{job.result().get\_statevector(qc)}. 
On the other hand, if the programmer decides to use an actual NISQ machine (which does not return a statevector) to run the circuit, they may not be able to use Cirquo's functionalities directly. However, they can use the noise model of the NISQ machine they used with the QASM simulator (and the slicer, if needed) to overcome that limitation.



The test generation functions Cirquo offers for the subroutines:
\begin{itemize}
    \item Quantum Full Adder.
    \item The Diffusion Operator.
    \item The W state.
    \item The GHZ state.
    \item The Dicke State.
    \item Quantum Fourier Transform (QFT).
    \item Quantum Phase Estimation (QPE).
\end{itemize}

The programmer can utilize Cirquo's implementation of these subroutines or use the testing aspect to test their implementation of these subroutines. For example, to test an implementation of the W state (the superposition of all states with Hamming weight 1), programmers can use Cirquo to generate tests for the W state based on the number of input qubits. The function to create tests for any of the subroutines works as follows: Given the number of input qubits, the function generates 6 basic inputs corresponding to the different bases $\{\vert0\rangle, \vert1\rangle\}$, $\{\vert+\rangle, \vert-\rangle\}$, and $\{\vert i\rangle, \vert-i\rangle\}$.\\
Returning to the example of generating tests for the W state, assume that we need to create tests for a 2-qubit W state. We can use the function \texttt{generate\_w\_state\_test\_cases(2)} to generate the tests in a format we can pass to the testing function to validate the correctness of a given W state implementation as shown in Listing~\ref{test_ws}.


\begin{lstlisting}[language=Python, caption=Test vectors for the 4-qubit W state., label=test_ws]
{
'name': 'test 0', 'input': [(1+0j), 0j, 0j, 0j], 'expected_output': [0j, (0.707+0j), (0.707+0j), 0j]
}
{
'name': 'test 1', 'input': [0j, 0j, 0j, (1+0j)], 'expected_output': [(-2.586e-17+0j), 0j, 0j, (1+0j)]
}
{
'name': 'test +', 'input': [(0.5+0j), (0.5+0j), (0.5+0j), (0.5+0j)], 'expected_output': [(0.5+0j), (0.707+0j), (-9.872e-17+0j), (0.5+0j)]
}
{
'name': 'test -', 'input': [(0.5+0j), (-0.5+0j), (-0.5+0j), (0.5+0j)], 'expected_output': [(-0.499+0j), (1.0751e-16+0j), (0.707+0j), (0.5+0j)]
}
{
'name': 'test i', 'input': [(0.5+0j), 0.5j, 0.5j, (-0.5+0j)], 'expected_output': [(1.2930e-17+0.5j), (0.353+0.353j), (0.353-0.353j), (-0.5-1.293e-17j)]
}
{
'name': 'test -i', 'input': [(0.5+0j), -0.5j, -0.5j, (-0.5+0j)], 'expected_output': [(1.293e-17-0.5j), (0.3535-0.353j), (0.353+0.353j), (-0.5+1.293e-17j)]}
]
\end{lstlisting} 

This list of tests can then be used with the \texttt{fQuantTester} to run tests on any implementation of the W state to validate its functionality. The W state only needs one parameter to be defined: the number of input qubits. However, some subroutines, namely the Dicke state, require two parameters to be defined: the number of qubits and the Hamming weight of the register. To generate the test vectors for a 3-qubit Dicke state with a Hamming weight of 2, we use the function \texttt{generate\_dicke\_state\_test\_cases(3,2)}.
%, which results in the tests in Listing.~\ref{test_ds}.
The general format of a test vector supported by Cirquo is shown in Listing~\ref{test_format}. When constructing tests for AP blocks, the \textit{input} and \textit{expected\_out} values could be a list of classical representations of the qubits. At the same time, they would be the state vector of the qubits when testing the AR and PM blocks.

\begin{lstlisting}[language=Python, caption=The format of test vectors., label=test_format]
test_cases = [
    {
        "name": "test 1",
        "input": [],
        "expected_output": []
    },
    .
    .
    .
    {
        "name": "test n",
        "input": [],
        "expected_output": []
    }
]
\end{lstlisting} 


Consider a simple amplitude redistribution circuit like a single-qubit Quantum Fourier Transform (QFT). The QFT can be represented as:

\begin{equation}
QFT|j\rangle = \frac{1}{\sqrt{2}}\sum_{k=0}^{1} e^{2\pi ijk / 2}|k\rangle
\end{equation}

where $j, k \in \{0, 1\}$ are the computational basis states.

To perform QPT on this circuit:

\begin{enumerate}
    \item Prepare the basis states $|0\rangle$ and $|1\rangle$.
    \item Apply the QFT to each state.
    \item Perform state tomography on the output states to obtain the transformed states.
    \item Reconstruct the process matrix $\chi$ to characterize the QFT operation.
\end{enumerate}

By analyzing $\chi$, one can determine if the QFT circuit accurately redistributes the amplitudes as expected or if there are errors that need debugging.


Consider a multi-quit amplitude redistribution circuit. Performing full QPT on such a circuit might be prohibitively complex. However, SPT can be applied selectively to those parts if the aim is to debug a specific gate or a set of gates within the circuit.

For example, in a circuit implementing a multi-qubit QFT, SPT can target only those gates if there's suspicion that a particular set of gates is malfunctioning. This selective focus allows for efficient debugging without reconstructing the entire process matrix for the whole circuit.



The steps for SPT are similar to QPT but are applied selectively:

\begin{enumerate}
    \item Identify the specific part of the circuit (e.g., a set of gates) to be analyzed.
    \item Prepare a set of input states that effectively probe the targeted part of the circuit.
    \item Apply the quantum process $\mathcal{E}$ to each state, ensuring only the selected part of the process contributes significantly to the transformation.
    \item Perform state tomography on the output states and reconstruct the relevant elements of the process matrix $\chi$.
\end{enumerate}



SPT provides a more practical approach for debugging large and complex quantum circuits. However, its effectiveness depends on accurately identifying the parts of the circuit that need debugging. Incorrect selection may lead to overlooking critical errors elsewhere in the circuit.

In summary, Selective Process Tomography offers a targeted and resource-efficient method for debugging specific elements within quantum circuits, particularly useful for amplitude redistribution circuits where complete process analysis is challenging.

\subsection{Testing Circuit blocks with unknown output}
Often, the case when testing and debugging quantum programs is that although we may know the expected results of the total circuit, we do not know the results of some (or all) of the slices. The programmer can refer to some common subroutines and some optimal test vectors to eliminate these subroutines as the cause of the error if any of them are included in the implemented algorithm. However, for those slices that are not one of those common subroutines, the programmer can use the basic test vectors to analyze the circuit's behavior. It is worth mentioning that the exploration test vectors are not intended to be the optimal test vectors for all circuits but rather a starting point for the programmer to observe the behavior of their program. 





%Due to that, we need to use other approaches to debug and test AR blocks. One method of doing that is through process tomography.

%%%%
%\COMMENT{ADD a paragraph about using the dagger if we want to test the whole circuit and then selective process tomo for a portion of the circuit.}

Quantum Process Tomography (QPT)~\cite{beck2012process, mohseni2008quantum} is a powerful tool for analyzing and debugging quantum circuits, particularly amplitude redistribution circuits. This method reconstructs the complete quantum process, represented by a superoperator, that a quantum state undergoes in a quantum circuit.

In QPT, the quantum process $\mathcal{E}$, acting on a quantum state $\rho$, is described by a completely positive trace-preserving (CPTP) map:

\begin{equation}
\mathcal{E}(\rho) = \sum_{m,n} \chi_{mn} E_m \rho E_n^\dagger
\end{equation}

Where $\{E_m\}$ are a set of basis operators for the system's Hilbert space, and $\chi_{mn}$ is the process matrix describing the process $\mathcal{E}$. The goal of QPT is to determine the matrix $\chi$ experimentally.


The procedure for QPT involves the following steps:

\begin{enumerate}
    \item Prepare a complete set of input states $\{\rho_i\}$.
    \item Apply the quantum process $\mathcal{E}$ to each state.
    \item Measure the output states using quantum state tomography to obtain $\mathcal{E}(\rho_i)$.
    \item Use the data to reconstruct the process matrix $\chi$.
\end{enumerate}


Though QPT can theoretically be a handy tool, it is costly to execute practically. Hence, we need a form of approximation and simplification to make it more practical. Since we use the slicer to form smaller circuits, we can use selective process tomography to test the smaller circuits or specific parts of a larger circuit.

Selective Process Tomography (SQPT)~\cite{bendersky2009selective, bendersky2008selective} is an advanced variant of Quantum Process Tomography (QPT) that focuses on a specific part of a quantum process. This technique is more practical in case of complex quantum circuits, where full-process tomography may be impractical due to many qubits and gates.


SQPT involves selectively reconstructing only some aspects of the process matrix $\chi$. This approach significantly reduces the experimental complexity and resources required, making it more feasible for large-scale quantum circuits.


\begin{figure}
\centering
\includegraphics[scale=0.2]{pics/ghz_cir.pdf}
\caption{A circuit for constructing a 3-qubit GHZ state.}
\label{3ghz}
\end{figure}

The process in SQPT can be described as follows:

\begin{equation}
\mathcal{E}_{\text{selective}}(\rho) = \sum_{m,n \in S} \chi_{mn} E_m \rho E_n^\dagger
\end{equation}

Where $S$ is a subset of indices chosen based on the specific elements of $\chi$ that are of interest.

Let us consider a simple example of how SQPT can be used as a debugging technique for AR blocks. The example we will think of is a 3-qubit GHZ circuit.
The GHZ state for a three-qubit system is given by:
\[ \frac{\ket{000} + \ket{111}}{\sqrt{2}} \]

To use process tomography, we need to consider the density matrix of the process we are trying to estimate. The density matrix of a 3-qubit GHZ \( \rho_{\text{GHZ}} \) is:
\[ \rho_{\text{GHZ}} = \frac{1}{2} \begin{pmatrix}
1 & 0 & 0 & 0 & 0 & 0 & 0 & 1 \\
0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
1 & 0 & 0 & 0 & 0 & 0 & 0 & 1 \\
\end{pmatrix} \]

The diagonal elements of this density represent probabilities of measuring the answers. In this case states $\vert000\rangle$ and $\vert111\rangle$. The sum of these two probabilities must be 1. At the same time, the off-diagonal elements indicate some level of quantum superposition or entanglement between the states.

We can either form a full QPT to obtain the entire density matrix or use selective process tomography to focus on a specific part of the matrix. 

For this example, let us focus on the top-left 2x2 block of the density matrix, which is:
\[ \rho_{\text{top-left}} = \frac{1}{2} \begin{pmatrix}
1 & 0 \\
0 & 0 \\
\end{pmatrix} \]

This portion of the matrix tells us information about states \( \ket{000} \) and \( \ket{001} \).

To perform SQPT, we must do selective measurements on the desired qubits.

Measure the \( \ket{000} \) state using the projector \( P_{000} = \ket{000}\bra{000} \). Which gives the probability \( p_{000} \).
Measure the \( \ket{001} \) state using the projector \( P_{001} = \ket{001}\bra{001} \). Which gives the probability \( p_{001} \). In this case, this should be zero.
The off diagonal terms of this small matrix \( \rho_{00,01} \) and \( \rho_{01,00} \) should also be zero.


The estimated top-left corner of the full-density matrix should be:
\[ \rho_{\text{top-left}} = \begin{pmatrix}
p_{000} & 0 \\
0 & 0 \\
\end{pmatrix} \]

In an ideal GHZ state, \( p_{000} \) should be close to 0.5. We can perform a simple form of this using the code in Listing~\ref{ghztest}.

\begin{lstlisting}[language=Python, caption=An Implementation of a simple SQPT test of a 3-qubit GHZ state using Qiskit., label=ghztest]
from qiskit import QuantumCircuit, execute, Aer

qc = QuantumCircuit(3, 3)

qc.append(ghz, [0,1,2])
qc.measure([0, 1, 2], [0, 1, 2])

simulator = Aer.get_backend('qasm_simulator')
result = execute(qc, simulator, shots=10000).result()
counts = result.get_counts(qc)

# Calculate the probability of observing '000'
prob_000 = counts.get('000', 0) / 10000
prob_001 = counts.get('001', 0)/ 10000

# The top-left corner of the density matrix
rho_top_left = [[prob_000, 0], [0, 0]]

# Print the results
print("Top-left corner of the density matrix:", rho_top_left)
\end{lstlisting}


Hence, if we have a block of a circuit implementing the GHZ state, we can execute it and measure the probabilities of the desired terms in the density matrix, which will give us information about whether or not a bug exists in the circuit.

It is worth mentioning that often, AR blocks are packaged subroutines, such as the GHZ state, W state, QFT, or even Grover's diffusion. Hence, programmers will not need to build it from scratch. However, if they do, they will have something to compare their results with, which will assist in the debugging process.


The simplification involves evaluating the exponential terms for each \(k\):

\begin{itemize}
    \item For \(k=0\): All terms sum to 4.
    \item For \(k=1, 3, 5, 7\) (odd \(k\)): The sum is 0 due to symmetry in the complex plane.
    \item For \(k=2, 6\): The terms sum to \(-4\) because \(e^{2\pi i \cdot j / 2}\) for odd \(j\) yields \(-1\).
    \item For \(k=4\): The sum is 4 because \(e^{2\pi i \cdot j}\) is 1 for any integer \(j\).
\end{itemize}

Therefore, the QFT-transformed state is:

==> dontuse-bibx.tex <==

% Generated by IEEEtran.bst, version: 1.12 (2007/01/11)
\begin{thebibliography}{10}
\providecommand{\url}[1]{#1}
\csname url@samestyle\endcsname
\providecommand{\newblock}{\relax}
\providecommand{\bibinfo}[2]{#2}
\providecommand{\BIBentrySTDinterwordspacing}{\spaceskip=0pt\relax}
\providecommand{\BIBentryALTinterwordstretchfactor}{4}
\providecommand{\BIBentryALTinterwordspacing}{\spaceskip=\fontdimen2\font plus
\BIBentryALTinterwordstretchfactor\fontdimen3\font minus
  \fontdimen4\font\relax}
\providecommand{\BIBforeignlanguage}[2]{{%
\expandafter\ifx\csname l@#1\endcsname\relax
\typeout{** WARNING: IEEEtran.bst: No hyphenation pattern has been}%
\typeout{** loaded for the language `#1'. Using the pattern for}%
\typeout{** the default language instead.}%
\else
\language=\csname l@#1\endcsname
\fi
#2}}
\providecommand{\BIBdecl}{\relax}
\BIBdecl


\bibitem{bennett73:reversible}Bennett, C. Logical Reversibility of Computation. {\em IBM J. Res. Develop.}. \textbf{17} pp. 525-532 (1973)
\bibitem{bennett88:_notes}Bennett, C. Notes on the history of reversible computation. {\em IBM J. Of Research And Development}. \textbf{32} (1988), reprinted in IBM J. R.\&D. Vol. 44 No. 1/2, Jan./Mar. 2000, pp. 270–277.
\bibitem{farhi2014quantum}Farhi, E., Goldstone, J. \& Gutmann, S. A quantum approximate optimization algorithm. {\em ArXiv Preprint ArXiv:1411.4028}. (2014)
\bibitem{gay05:_quant_progr_lang}Gay, S. Quantum Programming Languages: Survey and Bibliography. {\em Bulletin Of The European Association For Theoretical Computer Science}. (2005,6)
\bibitem{HOGG2000181}Hogg, T. \& Portnov, D. Quantum optimization. {\em Information Sciences}. \textbf{128}, 181 - 197 (2000), http://www.sciencedirect.com/science/article/pii/S0020025500000529
\bibitem{mcclean2016theory}McClean, J., Romero, J., Babbush, R. \& Aspuru-Guzik, A. The theory of variational hybrid quantum-classical algorithms. {\em New Journal Of Physics}. \textbf{18}, 023023 (2016)
\bibitem{mosca_et_al:DR:2019:10329}Mosca, M., Roetteler, M. \& Selinger, P. Quantum Programming Languages (Dagstuhl Seminar 18381). {\em Dagstuhl Reports}. \textbf{8}, 112-132 (2019), http://drops.dagstuhl.de/opus/volltexte/2019/10329
\bibitem{peruzzo2014variational}Peruzzo, A., McClean, J., Shadbolt, P., Yung, M., Zhou, X., Love, P., Aspuru-Guzik, A. \& O’Brien, J. A variational eigenvalue solver on a photonic quantum processor. {\em Nature Communications}. \textbf{5} (2014)
\bibitem{preskill:PH-CS219}Preskill, J. Lecture notes for PH/CS 219 at Caltech. (available on the web,2019), http://www.theory.caltech.edu/~preskill/ph219/index.html\#lecture
\bibitem{tip1995slicing}Tip, F. A survey of program slicing techniques. {\em Journal Of Programming Languages}. \textbf{3} pp. 121-189 (1995)
\bibitem{Trugenberger_2002}Trugenberger, C. Quantum optimization for combinatorial searches. {\em New Journal Of Physics}. \textbf{4} pp. 26-26 (2002,4), https://doi.org/10.1088%252F1367-2630%252F4%252F1%252F326
\bibitem{lampson1980processor}Lampson, B. \& Pier, K. A processor for a high-performance personal computer. {\em Proceedings Of The 7th Annual Symposium On Computer Architecture}. pp. 146-160 (1980)
\bibitem{sutor19:dancing}Sutor, R. Dancing with Qubits. (Packt Publishing,2019)
\bibitem{xu2005brief}Xu, B., Qian, J., Zhang, X., Wu, Z. \& Chen, L. A brief survey of program slicing. {\em ACM SIGSOFT Software Engineering Notes}. \textbf{30}, 1-36 (2005)
\bibitem{preskill2018quantum}Preskill, J. Quantum Computing in the NISQ era and beyond. {\em Quantum}. \textbf{2} pp. 79 (2018)
\bibitem{schuld2019evaluating}Schuld, M., Bergholm, V., Gogolin, C., Izaac, J. \& Killoran, N. Evaluating analytic gradients on quantum hardware. {\em Physical Review A}. \textbf{99}, 032331 (2019)
\bibitem{chong2017programming}Chong, F., Franklin, D. \& Martonosi, M. Programming languages and compiler design for realistic quantum hardware. {\em Nature}. \textbf{549}, 180-187 (2017)
\bibitem{bichsel2020silq}Bichsel, B., Baader, M., Gehr, T. \& Vechev, M. Silq: A high-level quantum language with safe uncomputation and intuitive semantics. {\em Proceedings Of The 41st ACM SIGPLAN Conference On Programming Language Design And Implementation}. pp. 286-300 (2020)
\bibitem{aleksandrowicz2019qiskit}Aleksandrowicz, G., Alexander, T., Barkoutsos, P., Bello, L., Ben-Haim, Y., Bucher, D., Cabrera-Hernández, F., Carballo-Franquis, J., Chen, A., Chen, C. \& Others Qiskit: An open-source framework for quantum computing.  (2019)
\bibitem{10.1145/3387940.3392184}Barbosa, L. Software Engineering for 'Quantum Advantage'. (Association for Computing Machinery,2020), https://doi.org/10.1145/3387940.3392184
\bibitem{ai2018}Google AI Cirq, a python framework for creating, editing, and invoking Noisy Intermediate Scale Quantum (NISQ) circuits.  (2018), https://github.com/quantumlib/Cirq
\bibitem{h2018}University of Melbourne QUI, a Quantum User Interface tool.  (2018), https://qui.research.unimelb.edu.au
\bibitem{pyq}Rigetti Computing PyQuil: Quantum programming in Python. , https://github.com/rigetti/pyquil
\bibitem{rand2018qwire}Rand, R., Paykin, J. \& Zdancewic, S. QWIRE practice: Formal verification of quantum circuits in Coq. {\em ArXiv Preprint ArXiv:1803.00699}. (2018)
\bibitem{grover1996fast}Grover, L. A fast quantum mechanical algorithm for database search. {\em Proceedings Of The Twenty-eighth Annual ACM Symposium On Theory Of Computing}. pp. 212-219 (1996)
\bibitem{10.1145/3527330}Paltenghi, M. \& Pradel, M. Bugs in Quantum Computing Platforms: An Empirical Study. {\em Proc. ACM Program. Lang.}. \textbf{6} (2022,4), https://doi.org/10.1145/3527330
\bibitem{10172716}Paltenghi, M. \& Pradel, M. MorphQ: Metamorphic Testing of the Qiskit Quantum Computing Platform. {\em 2023 IEEE/ACM 45th International Conference On Software Engineering (ICSE)}. pp. 2413-2424 (2023)
\bibitem{9951172}Metwalli, S. \& Van Meter, R. A Tool For Debugging Quantum Circuits. {\em 2022 IEEE International Conference On Quantum Computing And Engineering (QCE)}. pp. 624-634 (2022)
\bibitem{metwalli2020finding}Metwalli, S., Le Gall, F. \& Van Meter, R. Finding Small and Large k-Clique Instances on a Quantum Computer. {\em IEEE Transactions On Quantum Engineering}. (2020)
\bibitem{van-meter19:_quant_tweet_zen}Van Meter, R. A Quantum Computer Architecture tweetstorm.  (2019,9), https://doi.org/10.5281/zenodo.3496597
\bibitem{harrow2009quantum}Harrow, A., Hassidim, A. \& Lloyd, S. Quantum algorithm for linear systems of equations. {\em Physical Review Letters}. \textbf{103}, 150502 (2009)
\bibitem{padmanabhan1986uncertainty}Padmanabhan, T., Seshadri, T. \& Singh, T. Uncertainty principle and the quantum fluctuations of the schwarzschild light cones. {\em International Journal Of Modern Physics A}. \textbf{1}, 491-498 (1986)
\bibitem{brodsky1998quantum}Brodsky, S., Pauli, H. \& Pinsky, S. Quantum chromodynamics and other field theories on the light cone. {\em Physics Reports}. \textbf{301}, 299-486 (1998)
\bibitem{srivastva2017debugging}Srivastva, S. \& Dhir, S. Debugging approaches on various software processing levels. {\em 2017 International Conference Of Electronics, Communication And Aerospace Technology (ICECA)}. \textbf{2} pp. 302-306 (2017)
\bibitem{arulraj13apollo}Arulraj, J., Kim, T. \& Kang, W. APOLLO: Automatic Detection and Diagnosis of Performance Regressions in Database Systems. {\em Proceedings Of The VLDB Endowment}. \textbf{13}
\bibitem{di2021s}Di Luna, G., Italiano, D., Massarelli, L., Österlund, S., Giuffrida, C. \& Querzoni, L. Who’s debugging the debuggers? Exposing debug information bugs in optimized binaries. {\em Proceedings Of The 26th ACM International Conference On Architectural Support For Programming Languages And Operating Systems}. pp. 1034-1045 (2021)
\bibitem{liu2006statistical}Liu, C., Fei, L., Yan, X., Han, J. \& Midkiff, S. Statistical debugging: A hypothesis testing-based approach. {\em IEEE Transactions On Software Engineering}. \textbf{32}, 831-848 (2006)
\bibitem{mccauley2008debugging}McCauley, R., Fitzgerald, S., Lewandowski, G., Murphy, L., Simon, B., Thomas, L. \& Zander, C. Debugging: a review of the literature from an educational perspective. {\em Computer Science Education}. \textbf{18}, 67-92 (2008)
\bibitem{zheng2006statistical}Zheng, A., Jordan, M., Liblit, B., Naik, M. \& Aiken, A. Statistical debugging: simultaneous identification of multiple bugs. {\em Proceedings Of The 23rd International Conference On Machine Learning}. pp. 1105-1112 (2006)
\bibitem{NIELSEN2006147}Nielsen, M. Cluster-state quantum computation. {\em Reports On Mathematical Physics}. \textbf{57}, 147-161 (2006), https://www.sciencedirect.com/science/article/pii/S0034487706800145
\bibitem{10.1145/3445814.3446758}Tang, W., Tomesh, T., Suchara, M., Larson, J. \& Martonosi, M. CutQC: Using Small Quantum Computers for Large Quantum Circuit Evaluations. {\em Proceedings Of The 26th ACM International Conference On Architectural Support For Programming Languages And Operating Systems}. pp. 473-486 (2021), https://doi.org/10.1145/3445814.3446758
\bibitem{andrzejewski2007statistical}Andrzejewski, D., Mulhern, A., Liblit, B. \& Zhu, X. Statistical debugging using latent topic models. {\em European Conference On Machine Learning}. pp. 6-17 (2007)
\bibitem{montanaro2015:qualgo-qi}Montanaro, A. Quantum algorithms: an overview. {\em Npj Quantum Information}. \textbf{2} pp. 15023 (2016)
\bibitem{ladd10:_quantum_computers}Ladd, T., Jelezko, F., Laflamme, R., Nakamura, Y., Monroe, C. \& O'Brien, J. Quantum computers. {\em Nature}. \textbf{464} pp. 45-53 (2010,3)
\bibitem{Siraichi:2018:QA:3179541.3168822}Siraichi, M., Santos, V., Collange, S. \& Pereira, F. Qubit Allocation. {\em Proceedings Of The 2018 International Symposium On Code Generation And Optimization}. pp. 113-125 (2018), http://doi.acm.org/10.1145/3168822
\bibitem{nishio20:error-aware}Nishio, S., Pan, Y., Satoh, T., Amano, H. \& Van Meter, R. Extracting Success from IBM’s 20-Qubit Machines Using Error-Aware Compilation. {\em J. Emerg. Technol. Comput. Syst.}. \textbf{16} (2020,5), https://doi.org/10.1145/3386162
\bibitem{kotok1961dec}Kotok, A. DEC debugging tape. {\em Memo MIT-1 (rev.), MIT (Dec. 1961)}. (1961), https://www.computerhistory.org/pdp-1/189cc577e7b13aafbb0efab4c547d262/
\bibitem{Li}Li, G., Zhou, L., Yu, N., Ding, Y., Ying, M. \& Xie, Y. Projection-Based Runtime Assertions for Testing and Debugging Quantum Programs. {\em Proc. ACM Program. Lang.}. \textbf{4} (2020,11), https://doi.org/10.1145/3428218
\bibitem{miranskyy2021testing}Miranskyy, A., Zhang, L. \& Doliskani, J. On Testing and Debugging Quantum Software. {\em ArXiv Preprint ArXiv:2103.09172}. (2021)
\bibitem{huang2019statistical}Huang, Y. \& Martonosi, M. Statistical assertions for validating patterns and finding bugs in quantum programs. {\em Proceedings Of The 46th International Symposium On Computer Architecture}. pp. 541-553 (2019)
\bibitem{weder2020quantum}Weder, B., Barzen, J., Leymann, F., Salm, M. \& Vietz, D. The Quantum software lifecycle. {\em Proceedings Of The 1st ACM SIGSOFT International Workshop On Architectures And Paradigms For Engineering Quantum Software}. pp. 2-9 (2020)
\bibitem{cross2017open}Cross, A., Bishop, L., Smolin, J. \& Gambetta, J. Open quantum assembly language. {\em ArXiv Preprint ArXiv:1707.03429}. (2017)
\bibitem{heim2020quantum}Heim, B., Soeken, M., Marshall, S., Granade, C., Roetteler, M., Geller, A., Troyer, M. \& Svore, K. Quantum programming languages. {\em Nature Reviews Physics}. \textbf{2}, 709-722 (2020)
\bibitem{tannu2019mitigating}Tannu, S. \& Qureshi, M. Mitigating measurement errors in quantum computers by exploiting state-dependent bias. {\em Proceedings Of The 52nd Annual IEEE/ACM International Symposium On Microarchitecture}. pp. 279-290 (2019)
\bibitem{PhysRevX.8.031027}Endo, S., Benjamin, S. \& Li, Y. Practical Quantum Error Mitigation for Near-Future Applications. {\em Phys. Rev. X}. \textbf{8}, 031027 (2018,7), https://link.aps.org/doi/10.1103/PhysRevX.8.031027
\bibitem{PhysRevLett.119.180509}Temme, K., Bravyi, S. \& Gambetta, J. Error Mitigation for Short-Depth Quantum Circuits. {\em Phys. Rev. Lett.}. \textbf{119}, 180509 (2017,11), https://link.aps.org/doi/10.1103/PhysRevLett.119.180509
\bibitem{PhysRevX.7.021050}Li, Y. \& Benjamin, S. Efficient Variational Quantum Simulator Incorporating Active Error Minimization. {\em Phys. Rev. X}. \textbf{7}, 021050 (2017,6), https://link.aps.org/doi/10.1103/PhysRevX.7.021050
\bibitem{cruz2019efficient}Cruz, D., Fournier, R., Gremion, F., Jeannerot, A., Komagata, K., Tosic, T., Thiesbrummel, J., Chan, C., Macris, N., Dupertuis, M. \& Others Efficient quantum algorithms for ghz and w states, and implementation on the ibm quantum computer. {\em Advanced Quantum Technologies}. \textbf{2}, 1900015 (2019)
\bibitem{dicke1954coherence}Dicke, R. Coherence in spontaneous radiation processes. {\em Physical Review}. \textbf{93}, 99 (1954)
\bibitem{luo2022comprehensive}Luo, J., Zhao, P., Miao, Z., Lan, S. \& Zhao, J. A Comprehensive Study of Bug Fixes in Quantum Programs. {\em ArXiv Preprint ArXiv:2201.08662}. (2022)
\bibitem{ali2022}Ali, S., Yue, T. \& Abreu, R. When Software Engineering Meets Quantum Computing. {\em Commun. ACM}. \textbf{65}, 84-88 (2022,3), https://doi.org/10.1145/3512340
\bibitem{williams2014finding}Williams, V., Wang, J., Williams, R. \& Yu, H. Finding four-node subgraphs in triangle time. {\em Proceedings Of The Twenty-sixth Annual ACM-SIAM Symposium On Discrete Algorithms}. pp. 1671-1680 (2014)
\bibitem{le2014improved}Le Gall, F. Improved quantum algorithm for triangle finding via combinatorial arguments. {\em 2014 IEEE 55th Annual Symposium On Foundations Of Computer Science}. pp. 216-225 (2014)
\bibitem{castellanos2002triangle}Castellanos, J., Gómez, S. \& Guerra, V. The triangle method for finding the corner of the L-curve. {\em Applied Numerical Mathematics}. \textbf{43}, 359-373 (2002)
\bibitem{magniez2007quantum}Magniez, F., Santha, M. \& Szegedy, M. Quantum algorithms for the triangle problem. {\em SIAM Journal On Computing}. \textbf{37}, 413-424 (2007)
\bibitem{boyer1998tight}Boyer, M., Brassard, G., Høyer, P. \& Tapp, A. Tight bounds on quantum searching. {\em Fortschritte Der Physik: Progress Of Physics}. \textbf{46}, 493-505 (1998)
\bibitem{nielsen2002quantum}Nielsen, M. \& Chuang, I. Quantum computation and quantum information. (American Association of Physics Teachers,2002)
\bibitem{brassard2002quantum}Brassard, G., Hoyer, P., Mosca, M. \& Tapp, A. Quantum amplitude amplification and estimation. {\em Contemporary Mathematics}. \textbf{305} pp. 53-74 (2002)
\bibitem{green2013quipper}Green, A., Lumsdaine, P., Ross, N., Selinger, P. \& Valiron, B. Quipper: a scalable quantum programming language. {\em Proceedings Of The 34th ACM SIGPLAN Conference On Programming Language Design And Implementation}. pp. 333-342 (2013)
\bibitem{santos2016ibm}Santos, A. The IBM quantum computer and the IBM quantum experience. {\em ArXiv Preprint ArXiv:1610.06980}. (2016)
\bibitem{gidney}Gidney, C. Tools. {\em Algorithmic Assertions - Craig Gidney's Computer Science Blog}., https://algassert.com/
\bibitem{alexander2020qiskit}Alexander, T., Kanazawa, N., Egger, D., Capelluto, L., Wood, C., Javadi-Abhari, A. \& McKay, D. Qiskit pulse: programming quantum computers through the cloud with pulses. {\em Quantum Science And Technology}. \textbf{5}, 044006 (2020)
\bibitem{kissinger2019pyzx}Kissinger, A. \& Wetering, J. Pyzx: Large scale automated diagrammatic reasoning. {\em ArXiv Preprint ArXiv:1904.04735}. (2019)
\bibitem{booth2020qci}Booth, M., Berwald, J., Chukwu, U., Dawson, J., Dridi, R., Le, D., Wainger, M. \& Reinhardt, S. QCI Qbsolv delivers strong classical performance for quantum-ready formulation. {\em ArXiv Preprint ArXiv:2005.11294}. (2020)
\bibitem{murali2019full}Murali, P., Linke, N., Martonosi, M., Abhari, A., Nguyen, N. \& Alderete, C. Full-stack, real-system quantum computer studies: Architectural comparisons and design insights. {\em 2019 ACM/IEEE 46th Annual International Symposium On Computer Architecture (ISCA)}. pp. 527-540 (2019)
\bibitem{sivarajah2020t}Sivarajah, S., Dilkes, S., Cowtan, A., Simmons, W., Edgington, A. \& Duncan, R. t| ket>: a retargetable compiler for NISQ devices. {\em Quantum Science And Technology}. \textbf{6}, 014003 (2020)
\bibitem{zhao2021bugs4q}Zhao, P., Zhao, J., Miao, Z. \& Lan, S. Bugs4Q: A Benchmark of Real Bugs for Quantum Programs. {\em 2021 36th IEEE/ACM International Conference On Automated Software Engineering (ASE)}. pp. 1373-1376 (2021)
\bibitem{campos2021qbugs}Campos, J. \& Souto, A. Qbugs: A collection of reproducible bugs in quantum algorithms and a supporting infrastructure to enable controlled quantum software testing and debugging experiments. {\em 2021 IEEE/ACM 2nd International Workshop On Quantum Software Engineering (Q-SE)}. pp. 28-32 (2021)
\bibitem{PRXQuantum.3.010309}Eddins, A., Motta, M., Gujarati, T., Bravyi, S., Mezzacapo, A., Hadfield, C. \& Sheldon, S. Doubling the Size of Quantum Simulators by Entanglement Forging. {\em PRX Quantum}. \textbf{3}, 010309 (2022,1), https://link.aps.org/doi/10.1103/PRXQuantum.3.010309
\bibitem{VishVish}Badges, V. \& Badges I am getting “no memory for the experiment” error although I dont see any mistake. {\em Stack Overflow}. (2022,5), https://stackoverflow.com/questions/72413224/i-am-getting-no-memory-for-the-experiment-error-although-i-dont-see-any-mistak
\bibitem{Anita}Pandey, A. \& Wood, S. Import error when running Shor’s algorithm on Qiskit. {\em Stack Overflow}. (2023,6), https://stackoverflow.com/questions/76392444/import-error-when-running-shors-algorithm-on-qiskit
\bibitem{qsphere}qiskit.visualization.plot\_state\_qsphere. {\em Qiskit Documentation}. (2023,10), https://qiskit.org/documentation/stubs/qiskit.visualization.plot_state_qsphere


\end{thebibliography}
